Panoramic Structure from Motion via Geometric Relationship Detection

This paper addresses the problem of Structure from Motion (SfM) for indoor panoramic image streams, extremely challenging even for the state-of-the-art due to the lack of textures and minimal parallax. The key idea is the fusion of single-view and multi-view reconstruction techniques via geometric relationship detection (e.g., detecting 2D lines as coplanar in 3D). Rough geometry suffices to perform such detection, and our approach utilizes rough surface normal estimates from an image-to-normal deep network to discover geometric relationships among lines. The detected relationships provide exact geometric constraints in our line-based linear SfM formulation. A constrained linear least squares is used to reconstruct a 3D model and camera motions, followed by the bundle adjustment. We have validated our algorithm on challenging datasets, outperforming various state-of-the-art reconstruction techniques.

==> supplement_experiments.tex <==
% We would like to also emphasize that these evaluations
%are conducted on the best part of the OpenMVG reconstructions: OpenMVG
%failed to align many frames or reconstruct 3D structures that are not
%(cannot be) used in this evaluation.
Figures~\ref{fig:TestLivingRoom}-\ref{fig:TestAtrium} show the input
manual correspondences and the reprojected pixel locations of the
triangulated 3D point by our method (before or after the bundle
adjustment) and OpenMVG.
%
\begin{table}[!h]
		\caption{Quantitative evaluations on the camera matrices using reprojection errors.}
	\begin{center}
		\includegraphics[width=120mm]{figures/supp/quantitative.pdf}
	\end{center}
	\vspace{-0.3cm}

	\label{table:quantitative} \vspace{-0.2cm}
\end{table}

\begin{figure}[!t]
	\begin{center}
		\includegraphics[width=120mm]{figures/supp/TestLivingRoom1_0.pdf}
	\end{center}
	\vspace{-0.3cm}
	\caption{Reprojection error analysis in the {\it Living room} dataset.
 We have triangulated a 3D point from manual correspondences (yellow rectangles), then plot reprojected pixel coordinates based on the camera parameters of our method (before or after the bundle adjustment) and OpenMVG.}
 \label{fig:TestLivingRoom} \vspace{-0.2cm}
\end{figure}

\begin{figure}[!t]
	\begin{center}
		\includegraphics[width=120mm]{figures/supp/TestBedRoom1_0.pdf}
	\end{center}
	\vspace{-0.3cm}
 	\caption{Reprojection error analysis in the {\it Bed room} dataset.}
	\label{fig:TestBedRoom} \vspace{-0.2cm}
\end{figure}

\begin{figure}[!t]
	\begin{center}
		\includegraphics[width=120mm]{figures/supp/TestPlayRoom1_3.pdf}
	\end{center}
	\vspace{-0.3cm}
 	\caption{Reprojection error analysis in the {\it Play room} dataset.}
	\label{fig:TestPlayRoom} \vspace{-0.2cm}
\end{figure}

\begin{figure}[!t]
	\begin{center}
		\includegraphics[width=120mm]{figures/supp/TestTvRoom1_0.pdf}
	\end{center}
	\vspace{-0.3cm}
 	\caption{Reprojection error analysis in the {\it  Tv room} dataset.}
	\label{fig:TestTvRoom} \vspace{-0.2cm}
\end{figure}


\begin{figure}[!t]
	\begin{center}
		\includegraphics[width=120mm]{figures/supp/TestAtrium.pdf}
	\end{center}
	\vspace{-0.3cm}
	\caption{Reprojection error analysis in the {\it  Atrium} dataset.
 % We show input six images and three manual tracks (yellow rectangles),
 % reprojected points by our method before bundle adjustment (red cross),
 % our method after bundle adjustment (green cross) and OpenMVG (blue
% cross).
 }  \label{fig:TestAtrium} \vspace{-0.2cm}
\end{figure}


% slightly improved the accuracy of the geometry, however still
% problematic where OpenMVG still failed to recover the entire
% geometry. From the results, we could conclude that our coplanarity-based
% reconstruction contributes to recover more reasonable geometry of indoor
% Manhattan scenes.

% In the main manuscript, we showed the qualitative comparison against the
% OpenMVG. There, our method and openMVG used the same calibrated
% intrinsics parameters, however our method recovered the geometry using
% the refined rotation matrix from the IMU sensor (See Sec.4.1 in our main
% manuscript) while the openMVG directly estimated the rotations from the
% images. Therefore, it would be a natural question how the openMVG works
% when the rotation matrices from our methods are used. For answering this
% question, we ran OpenMVG using our refined rotation matrices and
% compared against the OpenMVG results.



% In this experiment, we only replaced the rotation matrices and unchanged
% other steps including the bundle adjustment in OpenMVG. The results were
% illustrated in Fig.\ref{fig:compOpenMVG}.

